Threshold-based Obfuscated Keys with Quantifiable Security against Invasive Readout

Advances in reverse engineering make it challenging to deploy any on-chip information in a way that is hidden from a determined attacker. A variety of techniques have been proposed for design obfuscation including look-alike cells in which functionality is determined by hard to observe mechanisms including dummy vias or transistor threshold voltages. Threshold-based obfuscation is especially promising because threshold voltages cannot be observed optically and require more sophisticated measurements by the attacker. In this work, we demonstrate the effectiveness of a methodology that applies threshold-defined behavior to memory cells, in combination with error correcting codes to achieve a high degree of protection against invasive reverse engineering. The combination of error correction and small threshold manipulations is significant because it makes the attacker's job harder without compromising the reliability of the obfuscated key. We present analysis to quantify key reliability of our approach, and its resistance to reverse engineering attacks that seek to extract the key through imperfect measurement of transistor threshold voltages. The security analysis and cost metrics we provide allow designers to make a quantifiable tradeoff between cost and security. We find that the combination of small threshold offsets and stronger error correcting codes are advantageous when security is the primary objective.

==> evaluation.tex <==
 In the next two sub-sections, first, we will evaluate the key reliability of our approach for different voltage offsets and with different error correcting codes and then, we will evaluate the key resistance against reverse engineering.
\subsection{Key reliability}
One of the important issues in key generation is the reliability of the key that is read on the output. Many undesirable phenomena such as environmental noise or voltage fluctuations affect the voltages that correspond to the key bits that are read on the output. Therefore, it is very common to have an error correcting scheme on the output to improve the reliability of the key values. One can improve the reliability of output key simply by using a higher threshold offset for transistors or using a more strong error correcting key values. However, each of these approaches come with its own drawbacks. Using a higher voltage offset makes reverse engineering easier and a better error correcting code comes with more expense in terms of area or power consumption. 
Based on the specifications of the design, a designer can choose from different options of voltage threshold offsets and key correcting codes to reach a certain amount of reliability that best suits the design.
\par
We focus on BCH codes, which is a class of codes that can be adapted for their block
size and the number of correctable errors in each block. We denote a certain BCH code as BCH[n, m, t]; where n is the block size, m is the size of useful data after error correction and t is the size of correctable errors in a block. If an error correcting code is able to correct t bits, the block fails if
more than t bits of error occur. Since we use the variable error rate model, the error rate of cells follow a random distribution instead of a single constant value.
We evaluated the key reliability for a 128-bit key using BCH codes of 255 bit blocks. 
\subsection{Key resistance against reverse engineering}
Since our method shares a single hidden key across multiple chips, a reverse engineer might benefit from analyzing multiple chips in order to reverse engineer the SRAM values and figure out the key.
Reliability of the reverse engineered key very much depends on the accuracy of the measurements. As of today, the reverse engineering of transistor threshold values is known to be a very hard task and the values obtained suffer from the lack of precision \todo[inline]{cite something here}. 

